Reinforcement Learning for Test Case Prioritization

Continuous Integration (CI) significantly reduces integration problems, speeds up development time, and shortens release time. However, it also introduces new challenges for quality assurance activities, including regression testing, which is the focus of this work. Though various approaches for test case prioritization have shown to be very promising in the context of regression testing, specific techniques must be designed to deal with the dynamic nature and timing constraints of CI. Recently, Reinforcement Learning (RL) has shown great potential in various challenging scenarios that require continuous adaptation, such as game playing, real-time ads bidding, and recommender systems. Inspired by this line of work and building on initial efforts in supporting test case prioritization with RL techniques, we perform here a comprehensive investigation of RL-based test case prioritization in a CI context. To this end, taking test case prioritization as a ranking problem, we model the sequential interactions between the CI environment and a test case prioritization agent as an RL problem, using three alternative ranking models. We then rely on carefully selected and tailored state-of-the-art RL techniques to automatically and continuously learn a test case prioritization strategy, whose objective is to be as close as possible to the optimal one. Our extensive experimental analysis shows that the best RL solutions provide a significant accuracy improvement over previous RL-based work, with prioritization strategies getting close to being optimal, thus paving the way for using RL to prioritize test cases in a CI context.

==> sections/defs.tex <==
%% FILENAME: defs.tex
%% AUTHOR:   Cameron Swords




%%------------------------------------------------------------------------
%% DEFINITION HELPERS
%%------------------------------------------------------------------------

\newcommand{\alt}{~~|~~}
\newcommand{\comp}[1]{\llbracket #1 \rrbracket}

\newcommand{\inlinexp}[1]{
{\footnotesize
 \[\begin{array}{l}
 #1
 \end{array}\]}}

\newcommand{\inlinexpa}[2]{
{\footnotesize
 \[\begin{array}{#1}
 #2
 \end{array}\]}}

\newcommand{\infr} [3] [] {\infer[\textsc{#1}]{#3}{#2}}
\newcommand{\iand}        {\qquad}

\newcommand{\Ctxt}       {\mathcal{E}}
\newcommand{\InCtxt} [1] {\Ctxt[#1]}

%%------------------------------------------------------------------------
%% REDUCTION RELATION MACROS
%%------------------------------------------------------------------------

\newcommand{\subst} [3]    {#3 [#2 / #1]}
\newcommand{\dstep} [2]    {#1 ~\Downarrow~ #2}

\newcommand{\ssosredex}        {\rightarrow}
\newcommand{\ctxtreduce}       {\mapsto}
\newcommand{\sstep}     [3] [] {#2 &\ssosredex&  #3 &\textsc{#1}}
\newcommand{\ctxtstep}  [3] [] {#2 &\ctxtreduce& #3 &\textsc{#1}}

%%------------------------------------------------------------------------
%% TYPE DEFINITION MACROS
%%------------------------------------------------------------------------

\newcommand{\funct} [2] {#1\nobreak\rightarrow\nobreak#2}
\newcommand{\boolt}     {\mathtt{bool}}

\newcommand{\typeEnv}         {\Gamma}
\newcommand{\entails}         {\vdash}
\newcommand{\judgment}   [3] {#1 \entails #2 : #3}
\newcommand{\envent}      [2] {\judgment{\typeEnv}{#1}{#2}}
\newcommand{\extenvent}   [4] {\judgment{\typeEnv, #1 : #2}{#3}{#4}}
\newcommand{\envlookup}   [3] {\infr{#1(#2) = #3}{\judgment{#1}{#2}{#3}}}

%%------------------------------------------------------------------------
%% EXPRESSION MACROS
%%------------------------------------------------------------------------

%% lambda
\newcommand{\lamdefe}  [2] {\lambda #1.~#2}
\newcommand{\lamdefea} [2] {\begin{array}{l}\lambda#1.\\\hspace*{.5em}#2\\\end{array}}

%% let
\newcommand{\letdefe}    [3] {\letbind{#1}{#2}~\letin{#3}}
\newcommand{\letdefarre} [3] {\begin{array}{l}\letbind{#1}{#2}\\\letin{#3})\\\end{array}}

\newcommand{\letbind}  [2] {\mathsf{let}~\lbind{#1}{#2}}
\newcommand{\letbindp} [2] {\mathsf{let}~(\lbind{#1}{#2})}
\newcommand{\lbind}    [2] {#1=#2}
\newcommand{\letin}    [1] {\mathsf{in}~#1}

%% if
\newcommand{\ife}      [3] {\ifline{#1}~\thenline{#2}~\elseline{#3}}
\newcommand{\ifea}     [3] {\begin{array}{l}\ifline{#1}\\\thenline{#2}\\\elseline{#3}\end{array}}

\newcommand{\ifop}         {\mathsf{if}}
\newcommand{\ifline}   [1] {\ifop~ #1}
\newcommand{\thenline} [1] {\mathsf{then}~#1}
\newcommand{\elseline} [1] {\mathsf{else}~#1}

%% opers
\newcommand{\binopdef}     {\mathit{binop}}
\newcommand{\unopdef}      {\mathit{unop}}
\newcommand{\binope}   [2] {\binopdef~#1~#2}
\newcommand{\unope}    [1] {\unopdef~#1}

\newcommand{\andop}        {\mathsf{and}}
\newcommand{\orop}         {\mathsf{or}}
\newcommand{\notop}        {\mathsf{not}}
\newcommand{\ande}     [2] {\mathsf{and}~#1~#2}
\newcommand{\ore}      [2] {\mathsf{or}~#1~#2}
\newcommand{\note}     [1] {\mathsf{not}~#1}

%% values
\newcommand{\falsev}     {\mathsf{false}}
\newcommand{\truev}      {\mathsf{true}}



==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this section, we discuss the limitations of our current implementation, most of which can be addressed as future work.



==> sections/helperfunctions.tex <==

\begin{table}
 \begin{threeparttable}
\centering
	\caption{Helper functions} 
	\label{tab:helperfunction}
    \begin{tabular}{|p{2.1cm}|p{6.1cm}|}
    %\toprule
    \hline
     \small \textbf{Function} &      \small \textbf{Description}  \\ 
    %\midrule
    \hline


         \hline
    \small \textit{out\_t($s$)}    & \small  returns outgoing transitions from state ${s}$.\\
     \hline
   
    
     \small \textit{parent($s$)}     & \small  returns the first-level container state of state ${s}$. %E.g.,  \textit{parent($s_{21}$)=\;\{$c_{2}$\}}. \\
    \\ \hline
    
   \small \textit{parents($s$)}     & \small returns all container states of state ${s}$. %E.g.,  \textit{parents($s_{21}$)=\;\{$c_{2},$ root(ABMSM)\}}. \\ 
    \\ \hline
   
    \textit{next\_s($s, \mathcal{H}$)}  & \small  (1) returns the last visited state inside state $s$ from history $\mathcal{H}$, (2) if (1) is unsuccessful (i.e., the state is active for the first time), returns the default state (initial state) inside $s$, and (3) if (1) and (2) are unsuccessful, returns $\emptyset$. \\ %E.g., if $\mathcal{H}=\emptyset$ then  \textit{next\_s($c_{11}, \mathcal{H})=\emptyset,$} and \textit{next\_s($ c_{12}, \mathcal{H})=in_{21}$}. \\
     \hline
    
     
    \textit{enabled($s$)} & \small  checks  state $s$ and its ancestors in bottom-up order, and returns the first (i.e., most deeply nested) outgoing transition, which can be triggered by the received message. It returns $\emptyset$ if no transition can be triggered. \\
     \hline 
   % \textit{up\_s($s,t$)}  & \small  returns $s$ and a subset of its parents in bottom-up order from state $s$ to the state that $t$ originated from. %E.g., \textit{up\_s($s_{12},t_{13}$)= $s_{12}$}. \\
   % \hline
    \textit{eval($ {E},g$)}   & \small  evaluates guard $g$ based on the values in  ${E}$ and returns the result. \\
    \hline
    
    \small  \textit{$msg_v($m$)$}    & \small accepts a message $m$ and returns a \textit{Boolean} variable $msg_v\_m$.  \\
    \hline

   \small \textit{payload($m$)}     & \small  accepts message $m$ and returns its payloads. %E.g.,  \textit{parent($s_{21}$)=\;\{$c_{2}$\}}. \\
    \\ \hline
    
    \textit{apply(${E},a_1 \dots a_n$)}   & \small executes a sequence of actions  $a_1 \dots a_n$ based on the values in $E$ and returns the updated $E$. \\
    \hline
    \end{tabular}
    %\begin{tablenotes}
    %  \small
    %  \item  	( \small $s$ is a state, $sm$ is an USM, $t$ is a transition, $\sigma$ is a configuration, $\mathcal{E}$ is mapping from variables to their values, $s_c$ is a composite state, $a_1 \dots a_n$ is a sequence of actions. )
%\end{tablenotes}

\end{threeparttable}
    \bigskip 
\end{table} 





==> sections/listwise-backup.tex <==

\begin{lstlisting}[mathescape=true,language=Python,caption={RL-based Listwise Ranking},label={code:listwise},frame=top,frame=bottom,frame=lines,morekeywords={Input,Output,bar,Function}, escapeinside={@}{@}] 
Input 
Let $T$ be a @set@ of test cases 
Let $s_o$ be the optimal ranking of $T$

Output 
$s_e$ an order (a sequence) of test cases in $T$ 

Let $rank$ be 0, done be False, @and@ reward be 0 
Let $obs$ be a vectorized  $T$  # observation space
Let $action$ be a vector of integer with @range@ [0,|$obs$|-1]
episode() # ref. Algorithm $\ref{code:rlflow}$

Function step($action$) # action is an array of ranks of test cases
    Let $sorted_t$ be the sorted test cases based on $action$ 
    calc_reward($sorted\_t$)  
    $done$ = True
    return $done$, $reward$, $obs$ 
        
Function calc_reward($sorted\_t$)   
 if $T$ contains a failed test case
    Let $apfd$ be the APFD of $sorted\_t$
    Let $apfd_{o}$ be the APFD of the optimal ranking of $T$
    return $\frac{apfd}{apfd_{o}}$ as reward
else
    return the NRPA of the $sorted\_t$ as reward
\end{lstlisting}
%\label{code:synth}

   % $reward$ = calc_reward($action$)
%    append obs[$index$] to $s_e$
 %   $obs$[$index$] = a dummy test case # mark the test case as selected
 %   if $rank$ < |$T$|-1
 %       $rank$ = $rank$ +1
 %   else
 %       $done$ = True
 %   return $done$, $reward$, $obs$ 
 
 
 \begin{lstlisting}[mathescape=true,language=Python,caption={RL-based Listwise Ranking},label={code:listwise},frame=top,frame=bottom,frame=lines,morekeywords={Input,Output,bar,Function}, escapeinside={@}{@}] 
Input 
Let $T$ be a @set@ of test cases 
Let $s_o$ be the optimal ranking of $T$

Output 
$s_e$ an order (a sequence) of test cases in $T$ 

Let $rank$ be 0, done be False, @and@ reward be 0 
Let $obs$ be a vectorized  $T$  # observation space
Let $action$ be an integer with @range@ [0,|$obs$|-1]
episode() # ref. Algorithm $\ref{code:rlflow}$

Function step($action$)
    $reward$ = calc_reward($action$)
    append obs[$index$] to $s_e$
    $obs$[$index$] = a dummy test case # mark the test case as selected
    if $rank$ < |$T$|-1
        $rank$ = $rank$ +1
    else
        $done$ = True
    return $done$, $reward$, $obs$ 
        
Function calc_reward($action$)   
 if $obs[action]$ is dummy: # previously selected or padded
    $reward$ = 0
 else
    $optimal\_rank$ = idx($s_o$,$obs[action]$)
    $reward$ = 1- (norm($optimal\_rank$) - norm($action$))^2

\end{lstlisting}
%\label{code:synth}

==> sections/pairwisewithmergesort.tex <==

\begin{lstlisting}[mathescape=true,language=Python,caption={RL-based Pairwise Ranking},label={code:pairwise},frame=top,frame=bottom,frame=lines,morekeywords={Input,Output,bar,Function}, escapeinside={@}{@}] 
Input 
Let $T$ be a @set@ of test cases 
Let $s_o$ be the optimal ranking of $T$

Output 
$s_e$ an order (a sequence) of test cases in $T$ 

Set sequence $s_e$ to a be random order of test cases in $T$
Let $idx_0$ be 0, $idx_1$ be 1, done be False, @and@ reward be 0
Let $obs$ be a vector [$s_e$[$idx_0$] , $s_e$[$idx_1$]] # a pair
episode()

Function step(action)
    
    
    
Function calc_reward(action)
    Let $sel\_test\_case$ be $obs[action]$ and $nonsel\_test\_case$ be  $obs[1- action]$
    if $sel\_test\_case.v$ > $nonsel\_test\_case.v$:
        reward = 1
    else if   $sel\_test\_case.v$ < $nonsel\_test\_case.v$::
        reward = 0
    else if $sel\_test\_case$.e <= $nonsel\_test\_case.e$:
        reward = 0.5
    else 
        reward = 0

\end{lstlisting}


==> sections/tables/features.tex <==

\begin{table}[t!]
\centering
	\caption{Code-base Features} 
	%\vspace{-.3cm}
	\label{tab:helperfunction2}
    \begin{tabular}{|p{3cm}|p{5cm}|}
    %\toprule
    \hline
     \small \textbf{Feature} &      \small \textbf{Description}  \\ 
    %\midrule
    \hline
        \small Bug probability of changes (BP) & \small   
 \\
     \hline
        \small Text/content similarity score (TS) & \small   
 \\
     \hline
      \small Static analysis based coverage (SA) & \small   
 \\
     \hline
     
        \small Evolution based coverage  (EC) & \small   
 \\
     \hline
     
      \small Complexity of changes  (CC) & \small   
 \\
     \hline
    \end{tabular}
   % \vspace{-.5cm}
\end{table} 

==> sections/tables/functionHelper.tex <==

\begin{table}[t!]
\centering
	\caption{Helper functions} 
	\vspace{-.3cm}
	\label{tab:helperfunction}
    \begin{tabular}{|p{1.1cm}|p{7cm}|}
    %\toprule
    \hline
     \small \textbf{Function} &      \small \textbf{Description}  \\ 
    %\midrule
    \hline

     \small \codee{$ra(a,ts)$}   &\small   returns  the rank assigned to ts by action a (the lower the rank, the higher the priority for the execution)
  \\
   
     \hline
   
   \small \codee{$ex(ts)$}     & \small   returns the execution time of test case ts \\
     \hline
  
    \end{tabular}
    \vspace{-.5cm}
\end{table} 





==> sections/tables/result-avg.tex <==
\begin{table*}[t]

\begin{center}
\begin{tabular}{ l|ccccccccccccccccccccccccc } 
\hline
\multicolumn{1}{c|}{\textbf{SB}} & \multicolumn{1}{c}{\textbf{FM}} & 
\multicolumn{2}{c}{\small \textbf{A2C}} & 
\multicolumn{2}{c}{\small \textbf{ACER} }& 
\multicolumn{2}{c}{\small \textbf{PPO}} & 
\multicolumn{2}{c}{\small \textbf{TRPO}} & 
\multicolumn{2}{c}{\small \textbf{DQN}} & 
\multicolumn{2}{c}{\small \textbf{DDPG}} & 
\multicolumn{2}{c}{\small \textbf{TD3}} & 
\multicolumn{2}{c}{\small \textbf{SAC}} \\
& & \small APFD & \small NRPA &  
\small APFD & \small NRPA  & 
\small APFD & \small NRPA  & 
\small APFD & \small NRPA  & 
\small APFD & \small NRPA  & 
\small APFD & \small NRPA  & 
\small APFD & \small NRPA  & 
\small APFD & \small NRPA   
\\
\hline
\hline

%'paintcontrol','POINTWISE','A2C','0.7563460495072359','0.5703532519597659','0.8979828281847287','0.0035633111137611875'
%'paintcontrol','POINTWISE','ACKTR','0.7477510769834939','0.5712844425521818','0.8979828281847287','0.00337145649835424'
%'paintcontrol','POINTWISE','DDPG','0.7460172056394558','0.5633495190893214','0.8979828281847287','0.003327909380469097'
%'paintcontrol','POINTWISE','PPO1','0.7471860741992532','0.5735048847441688','0.8979828281847287','0.0034850165741075402'
%'paintcontrol','POINTWISE','PPO2','0.7471921777511521','0.5715773804572609','0.8979828281847287','0.003374973923687099'
%'paintcontrol','POINTWISE','SAC','0.7477920900268612','0.5709816247238807','0.8979828281847287','0.0034476042684457205'
%'paintcontrol','POINTWISE','TD3','0.7467850748798739','0.5742008292807463','0.8979828281847287','0.0037521525340012247'
%'paintcontrol','POINTWISE','TRPO','0.7530015767046068','0.5732671933095662','0.8979828281847287','0.0035071771268796433'
%'paintcontrol','PAIRWISE','A2C','0.947436884686771','0.6679688568746173','0.8979828281847287','0.0030981431168280635'


\multirow{3}{.25cm}{\small \textbf{PC}}  
& \small \textbf{PO} & a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{LW}  & a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR} &  a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC   \\  
\hline

\multirow{3}{.2cm}{\small \textbf{IF}}  
& \small \textbf{PO} & a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{LW}  & a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR} &  a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC   \\  
\hline

\multirow{3}{.2cm}{\small \textbf{GS}}  
& \small \textbf{PO} & a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{LW}  & a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR} &  a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC   \\  
\hline

%'codec','POINTWISE','A2C','0.876405966143342','0.0000','0.0000','0.06810247654934934'
%'codec','POINTWISE','TD3','0.7622977140077897','0.0000','0.0000','0.0904781284518555'
%'codec','POINTWISE','DDPG','0.8781958699998801','0.0000','0.0000','0.08589066975231717'
%'codec','POINTWISE','ACKTR','0.7780693545942086','0.0000','0.0000','0.0818893195751267'
%'codec','POINTWISE','PPO2','0.8815900872119975','0.0000','0.0000','0.06612609307956441'
%'codec','POINTWISE','TRPO','0.8921712706041826','0.0000','0.0000','0.07478947727786897'
%'codec','POINTWISE','PPO1','0.8897078981628861','0.0000','0.0000','0.0763515354804607'
%'codec','POINTWISE','SAC','0.7802387873978038','0.0000','0.0000','0.09803607737123973'
%'codec','PAIRWISE','A2C','0.8846866291904859','0.0000','0.0000','0.11622149846496566'
%'codec','PAIRWISE','ACER','0.8986963146884704','0.0000','0.0000','0.11411180427828053'
%'codec','PAIRWISE','ACKTR','0.853862456253368','0.0000','0.0000','0.13385979958305866'
%'codec','PAIRWISE','DQN','0.875806033705512','0.0000','0.0000','0.11838606998471493'
%'codec','PAIRWISE','PPO1','0.8895029435186586','0.0000','0.0000','0.11704015807618219'
%'codec','PAIRWISE','PPO2','0.8802101480052759','0.0000','0.0000','0.11781995629696926'
%'codec','PAIRWISE','TRPO','0.86776402576406','0.0000','0.0000','0.12320508836661283'


\multirow{3}{.2cm}{\small \textbf{CO}}  
& \small \textbf{PO} & \small NA & \small 0.876 $\pm$ .06 & \small NA & \small NA & \small NA & 0.889 $\pm$ 0.11 & \small NA & \textbf{.892 $\pm$ .07 } &  \small NA  & \small NA & \small NA & \small .878 $\pm$ .08 & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR}  & \small NA & \small .884 $\pm$ .11 & \small NA & \textbf{.898$\pm$.11 $\star$ } & \small NA & \small .889 $\pm$ .11 & \small NA & .867$\pm$ .11  &  \small NA  & \small .875$\pm$0.11 & \small NA & \small NA & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{LW} &  a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC   \\  
\hline

%'imaging','POINTWISE','TRPO','0.8267717849557026','0.0069','0.0138','0.0035022976310014973'
%'imaging','POINTWISE','TD3','0.783024568839598','0.0069','0.0138','0.004981871011893138'
%'imaging','POINTWISE','SAC','0.7801579458453408','0.0138','0.0138','0.005388194385234125'
%'imaging','POINTWISE','PPO2','0.8536281682079339','0.0000','0.0138','0.0038827348326094012'
%'imaging','POINTWISE','PPO1','0.898858201536362','0.0000','0.0138','0.0026894357359938245'
%'imaging','POINTWISE','DDPG','0.8518723492237837','0.0069','0.0138','0.007919665889205361'
%'imaging','POINTWISE','ACKTR','0.7793579032320042','0.0069','0.0138','0.005516607289267836'
%'imaging','POINTWISE','A2C','0.8998880980983599','0.0069','0.0138','0.003344582969685964'
%'imaging','PAIRWISE','A2C','0.9029153601866416','0.0138','0.0138','0.01039512703277924'
%'imaging','PAIRWISE','ACER','0.9064341460662808','0.0138','0.0138','0.009638567582997873'
%'imaging','PAIRWISE','ACKTR','0.8717891543416649','0.0138','0.0138','0.010984584971992327'
%'imaging','PAIRWISE','DQN','0.8934580153659293','0.0138','0.0138','0.012074088219846858'
%'imaging','PAIRWISE','PPO1','0.8925279352398443','0.0138','0.0138','0.01091278411265179'
%'imaging','PAIRWISE','PPO2','0.8964977865421094','0.0138','0.0138','0.009983274598563218'
%'imaging','PAIRWISE','TRPO','0.8791217368907068','0.0069','0.0138','0.010859751938808176'



\multirow{3}{.2cm}{\small \textbf{IM}} 
& \small \textbf{PO} & NA & \textbf{.899$\pm$ .003} & \small NA & \small NA & \small NA & .898$\pm$ .002 & \small NA & .826$\pm$ .0073  &  \small NA  & \small NA & \small NA & \small .851$\pm$ .007 & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR}  & NA & \small .902$\pm$ .010 & \small NA & \textbf{.906$\pm$ .009} & \small NA & .896$\pm$ .009 & \small NA & .879$\pm$ .010 &  \small NA  & \small .893$\pm$ .012 & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{LW} &  a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC   \\  
\hline


%'imaging','POINTWISE','TRPO','0.8267717849557026','0.0069','0.0138','0.0035022976310014973'
%'imaging','POINTWISE','TD3','0.783024568839598','0.0069','0.0138','0.004981871011893138'
%'imaging','POINTWISE','SAC','0.7801579458453408','0.0138','0.0138','0.005388194385234125'
%'imaging','POINTWISE','PPO2','0.8536281682079339','0.0000','0.0138','0.0038827348326094012'
%'imaging','POINTWISE','PPO1','0.898858201536362','0.0000','0.0138','0.0026894357359938245'
%'imaging','POINTWISE','DDPG','0.8518723492237837','0.0069','0.0138','0.007919665889205361'
%'imaging','POINTWISE','ACKTR','0.7793579032320042','0.0069','0.0138','0.005516607289267836'
%'imaging','POINTWISE','A2C','0.8998880980983599','0.0069','0.0138','0.003344582969685964'
%'imaging','PAIRWISE','A2C','0.9029153601866416','0.0138','0.0138','0.01039512703277924'
%'imaging','PAIRWISE','ACER','0.9064341460662808','0.0138','0.0138','0.009638567582997873'
%'imaging','PAIRWISE','ACKTR','0.8717891543416649','0.0138','0.0138','0.010984584971992327'
%'imaging','PAIRWISE','DQN','0.8934580153659293','0.0138','0.0138','0.012074088219846858'
%'imaging','PAIRWISE','PPO1','0.8925279352398443','0.0138','0.0138','0.01091278411265179'
%'imaging','PAIRWISE','PPO2','0.8964977865421094','0.0138','0.0138','0.009983274598563218'
%'imaging','PAIRWISE','TRPO','0.8791217368907068','0.0069','0.0138','0.010859751938808176'



\multirow{3}{.25cm}{\small \textbf{IO}}  
& \small \textbf{PO} & NA & \small .826$\pm$ .003 & \small NA & \small NA & \small NA &  \textbf{.898 $\pm$ .002} & \small NA & .826$\pm$.003 &  \small NA  & \small NA & \small NA & \small .851$\pm$.007 & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR}  & NA & \small .902$\pm$.01 & \small NA &  \textbf{.906$\pm$.00} $\star$ & \small NA  & .896$\pm$.009 & \small NA & .879$\pm$.01  &  \small NA  & \small .892$\pm$.01 & \small NA & \small NA & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{LW} &  a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC   \\  
\hline

%'math','POINTWISE','A2C','0.8173609035845993','0.0370','0.1296','0.0028984232350710354'
%'math','POINTWISE','ACKTR','0.7784294791765278','0.0926','0.1296','0.0035786357265364384'
%'math','POINTWISE','DDPG','0.854131739465655','0.0556','0.1296','0.004097201045518614'
%'math','POINTWISE','PPO1','0.8225240216833244','0.0370','0.1296','0.002718041181676543'
%'math','POINTWISE','PPO2','0.8303367400021898','0.0185','0.1296','0.0022880426446904574'
%'math','POINTWISE','SAC','0.7778219423891292','0.0556','0.1296','0.004738225089696514'
%'math','POINTWISE','TD3','0.7705510014985939','0.0926','0.1296','0.0041163196865446235'
%'math','POINTWISE','TRPO','0.8217761729345383','0.0556','0.1296','0.002410266628338784'
%'math','PAIRWISE','A2C','0.8917480013874146','0.0556','0.1296','0.00894349335798235'
%'math','PAIRWISE','ACER','0.9070688725206553','0.0556','0.1296','0.008834661673929756'
%'math','PAIRWISE','ACKTR','0.8923282396512303','0.0185','0.1296','0.008664491899575695'
%'math','PAIRWISE','PPO1','0.8984919040702808','0.0926','0.1296','0.009648901572418246'
%'math','PAIRWISE','PPO2','0.8853428880614708','0.0926','0.1296','0.00964567083630434'
%'math','PAIRWISE','TRPO','0.9004879144945959','0.0556','0.1296','0.007981778418359868'



\multirow{3}{.2cm}{\small \textbf{MA}} 
& \small \textbf{PO} & NA & \small .817$\pm$.002 & \small NA & \small NA & \small NA & .830$\pm$.002 & \small NA & .821$\pm$.002 &  \small NA  & \small NA & \small NA & \textbf{.854$\pm$.004} & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR}  & NA & \small .891$\pm$.008 & \small NA & \textbf{.907$\pm$.008} & \small NA & .898$\pm$.009 & \small NA & .900$\pm$.007 &  \small NA  & \small .???$\pm$.00 & \small NA & \small NA & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{LW} &  a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC   \\  
\hline

%'Compress','POINTWISE','A2C','0.9001867994472827','0.0161','0.0161','0.0020822879111503352'
%'Compress','POINTWISE','PPO2','0.867167982484454','0.0138','0.0161','0.0027211788036417862'
%'Compress','POINTWISE','SAC','0.7709141880138921','0.0115','0.0161','0.005405702800553198'
%'Compress','POINTWISE','ACKTR','0.7742314398465407','0.0092','0.0161','0.003411829892206641'
%'Compress','POINTWISE','PPO1','0.9019747798988126','0.0115','0.0161','0.0016337882691324541'
%'Compress','POINTWISE','DDPG','0.7735966322478283','0.0092','0.0161','0.003263908240940795'
%'Compress','POINTWISE','TD3','0.7670513983828104','0.0092','0.0161','0.005743368795318624'
%'Compress','POINTWISE','TRPO','0.8995127562937066','0.0161','0.0161','0.0015666246030393248'
%'Compress','PAIRWISE','A2C','0.9241507373840292','0.0138','0.0161','0.00494936830473003'
%'Compress','PAIRWISE','ACER','0.9279070839737966','0.0092','0.0161','0.005049185281247495'
%'Compress','PAIRWISE','ACKTR','0.7327806040586821','0.0115','0.0161','0.005217086945839218'
%'Compress','PAIRWISE','DQN','0.9100996075568765','0.0181','0.0211','0.005279945927180713'
%'Compress','PAIRWISE','PPO1','0.922327068937744','0.0138','0.0161','0.004986026843030699'
%'Compress','PAIRWISE','PPO2','0.92210331295357','0.0138','0.0161','0.00490319878756868'
%'Compress','PAIRWISE','TRPO','0.915529506949719','0.0138','0.0161','0.0050901019905312105'



\multirow{3}{.33cm}{\small \textbf{CM}}  
& \small \textbf{PO} & NA & \small .900$\pm$.00 & \small NA & \small NA & \small NA & \textbf{.901$\pm$.00} & \small NA & \small .899$\pm$.00 &  \small NA  & \small NA & NA & \small .773$\pm$.00 & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR}  & \small NA & \small .924$\pm$.00 & \small NA & \textbf{.927$\pm$.00} $\star$ & \small NA & .922$\pm$00 & \small NA & \small .915$\pm$.00 &  \small NA  & \small .910$\pm$.00 & \small NA & \small NA & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{LW} &  a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC   \\  
\hline

%'lang','POINTWISE','A2C','0.8281537801601192','0.0000','0.0067','0.004862680266238337'
%'lang','POINTWISE','ACKTR','0.775025137021569','0.0067','0.0067','0.0033306910768257465'
%'lang','POINTWISE','DDPG','0.7746368749150184','0.0067','0.0067','0.003361603787514533'
%'lang','POINTWISE','PPO1','0.8535026673093411','0.0067','0.0067','0.0030870179820156655'
%'lang','POINTWISE','PPO2','0.8514605985170328','0.0000','0.0067','0.004080639732389583'
%'lang','POINTWISE','SAC','0.7804901809138032','0.0033','0.0067','0.004986886115996161'
%'lang','POINTWISE','TD3','0.7712613012846699','0.0067','0.0067','0.005081540041763426'
%'lang','POINTWISE','TRPO','0.8382650137616298','0.0067','0.0067','0.002933177264737076'
%'lang','PAIRWISE','A2C','0.8917642335593766','0.0000','0.0067','0.006969618696201484'
%'lang','PAIRWISE','ACER','0.9034568646382178','0.0033','0.0067','0.006877041211054438'
%'lang','PAIRWISE','ACKTR','0.8723693986684459','0.0067','0.0067','0.008886559208904398'
%'lang','PAIRWISE','DQN','0.8934424434283829','0.0073','0.0146','0.007366584629557501'
%'lang','PAIRWISE','PPO1','0.8839033426951352','0.0000','0.0067','0.007252419225067264'
%'lang','PAIRWISE','PPO2','0.8834215455660172','0.0000','0.0067','0.007342653658910377'
%'lang','PAIRWISE','TRPO','0.892006049869941','0.0000','0.0067','0.007118852286567901'



\multirow{3}{.2cm}{\small \textbf{LN}}  
& \small \textbf{PO} & NA & \small .820$\pm$.00 & \small NA & \small NA & \small NA & \textbf{.853$\pm$.00} & \small NA & .838$\pm$.00 &  \small NA  & \small NA & \small NA & \small .774$\pm$.00 & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR}  & NA & \small .891$\pm$.00 & \small NA & \textbf{.903$\pm$.00} $\star$ & \small NA & .883$\pm$.00 & \small NA & .892$\pm$.00 &  \small NA  & \small .0893$\pm$.00 & \small NA & \small NA & \small TD3 & \small TD3 & \small SAC & \small SAC    \\ 

& \small \textbf{PR} &  a2c & \small a2c & \small ACER & \small ACER & \small PPO & PPO & \small TRPO & TRPO &  \small DQN  & \small DQN & \small DDPG & \small DDPG & \small TD3 & \small TD3 & \small SAC & \small SAC   \\  
\hline
\hline



\end{tabular}
\end{center}

\end{table*}

==> sections/tables/trainingtime-backup.tex <==














%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[t]
\caption{The sum of training and testing time (Minutes) of all cycles of subjects in different configurations.}
\label{tab:results-training}
\begin{center}
\begin{tabular}{ p{.9cm}|cccccccccccccccccc} 
\hline
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c}{\small \textbf{RM}} & 
\multicolumn{2}{c}{\small \textbf{Paint.}} & 
\multicolumn{2}{c}{\small \textbf{IOFROL} }& 
%\multicolumn{1}{c}{\small \textbf{GTS}} & 
\multicolumn{2}{c}{\small \textbf{CODEC}} & 
\multicolumn{2}{c}{\small \textbf{IMAG}} & 
\multicolumn{2}{c}{\small \textbf{IO}} & 
\multicolumn{2}{c}{\small \textbf{COMP}} & 
\multicolumn{2}{c}{\small \textbf{LANG}} &
\multicolumn{2}{c}{\small \textbf{MATH}}  
%\multicolumn{2}{c}{\small \textbf{Comp. T}} 
\\
& & 
\small (Tr.) & \small (Pr.) &
\small (Tr.) & \small (Pr.) &

\small (Tr.) & \small (Pr.) &
\small (Tr.) & \small (Pr.) & 
\small (Tr.) & \small (Pr.) &
\small (Tr.) & \small (Pr.) &
\small (Tr.) & \small (Pr.) &
\small (Tr.) & \small (Pr.) 
%\small (Tr.)  &
%\small (Pr.)  &
\\
\hline
\hline




\multirow{2}{.40cm}{\small \textbf{A2C}}  
& \small \textbf{PO}
& \small 113.30& \small 3.5 
& \small 120.4& \small 2.3
& \small 38.4& \small 1.8
& \small 24.6& \small 1.3
& \small 41.0& \small 1.6
& \small 185.3& \small 4.4
& \small 90.4& \small 2.9
& \small 14.6& \small 0.5 \\ 

& \small \textbf{PR} 
& \small 1,227.7& \small 5.0
& \small 1,668.3& \small 4.5
& \small 70.3& \small 1.8
& \small 166.4& \small 1.6
& \small 196.3& \small 2.0
& \small 473.5& \small 4.5
& \small 476.6& \small 3.4
& \small 309.1& \small 0.7  \\

& \small \textbf{LW} 
& \small 723.5 & \small 14.2
& \small 1,234.3 & \small 33.9
& \small 102.3 & \small 2.6
& \small 117.5& \small 2.8
& \small 107.1& \small 4.5
& \small 563.1& \small 10.7
& \small 333.7& \small 7.1
& \small 280.8 & \small 3.0 \\
\hline

\multirow{2}{{.7cm}}{\small \textbf{ACER}}  
& \small \textbf{PR} 
& \small 1,118.2 & \small 9.1
& \small 1,418.5 & \small 6.7
& \small 49.8& \small 4.0
& \small 126.7 & \small 3.4
& \small 163.2 & \small 4.3
& \small 380.4 & \small 9.6
& \small 371.6 & \small 7.3
& \small 204.5 & \small 1.4 \\

& \small \textbf{LW} 
& \small 291.6 & \small 21.5
& \small 861.8 & \small 35.6
& \small 74.2 & \small 4.8
& \small 89.4 & \small 9.0
& \small 173.7 & \small 6.8
& \small 279.8 & \small 17.8
& \small 179.2 & \small 13.3
& \small 112.7 & \small 4.7 \\

\hline

\multirow{3}{{.7cm}}{\small \textbf{PPO1}}  
& \small \textbf{PO} 
& \small 122.0& \small 3.6 
& \small 72.2& \small 2.2
& \small 48.2& \small 1.9
& \small 25.6& \small 1.5
& \small 60.2& \small 1.9
& \small 224.8& \small 4.6
& \small 111.9& \small 3.1
& \small 7.5& \small 0.6 \\

& \small \textbf{PR} 
& \small 814.6& \small 5.0 
& \small 898.4& \small 3.7
& \small 56.0& \small 2.0
& \small 81.6& \small 1.8 
& \small 122.4& \small 2.1
& \small 348.8& \small 4.7
& \small 265.7& \small 3.7
& \small 172.2& \small 0.8 \\

& \small \textbf{LW} 
& \small 241.7 & \small 62.5
& \small 502.8 & \small 144.3
& \small 53.3 & \small 4.8
& \small 51.5 & \small 8.9
& \small 87.2 & \small 6.9
& \small 287.1 & \small 21.7
& \small 201.4 & \small 72.6
& \small 97.6 & \small 18.9 \\

\hline


\multirow{3}{{.7cm}}{\small \textbf{PPO2}}  
& \small \textbf{PO} 
& \small 122.1& \small 3.6 
& \small 72.2& \small 2.2
& \small 48.2& \small 1.9
& \small 60.2& \small 1.9 
& \small 25.6& \small 1.5 
& \small 224.8& \small 4.6
& \small 111.9& \small 3.1
& \small 7.5& \small 0.6 \\

& \small \textbf{PR}
& \small 814.6& \small 5.0
& \small 898.4& \small 3.7
& \small 56.0 & \small 2.0
& \small 232.2& \small 43.6
& \small 122.4& \small 2.1
& \small 348.8& \small 4.7
& \small 265.7& \small 3.7
& \small 172.2& \small 0.8 \\

& \small \textbf{LW} 
& \small 418.2 & \small 34.1
& \small 303.8 & \small 100.6
& \small 68.7 & \small 3.2
& \small 73.2 & \small 4.9
& \small 95.5 & \small 7.8
& \small 534.0 & \small 26.1
& \small 320.9 & \small 25.7 
& \small 115.0 & \small 10.9 \\

\hline


\multirow{3}{{.7cm}}{\small \textbf{TRPO}}  
& \small \textbf{PO} 
& \small 117.6& \small 6.8 
& \small 74.6& \small 4.3
& \small 29.6& \small 4.0
& \small 23.4& \small 2.8
& \small 56.9& \small 3.5
& \small 245.2& \small 9.1
& \small 94.0 & \small 6.1
& \small 11.1 & \small 1.1 \\

& \small \textbf{PR} 
& \small 631.8& \small 6.8 
& \small 761.7& \small 5.2
& \small 69.6& \small 3.2
& \small 77.4& \small 2.7
& \small 108.9& \small 3.4
& \small 344.7& \small 7.5
& \small 285.8& \small 6.2
& \small 170.5& \small 1.2 \\

& \small \textbf{LW} 
& \small 196.3 & \small 175.2
& \small 570.0 & \small 77.3
& \small 96.4 & \small 3.4
& \small 53.9 & \small 4.4
& \small 55.8 & \small 5.9
& \small 445.5 & \small 22.1
& \small 170.8 & \small 160.3 
& \small 108.8 & \small 9.5 \\
\hline





\multirow{2}{{.7cm}}{\small \textbf{DQN}}
& \small \textbf{PR} 
& \small 5,021.3 & \small 5.7
& \small 3,356.3 & \small 4.4
& \small 104.5& \small 2.4
& \small 501.3& \small 2.3
& \small 675.9& \small 2.8 
& \small 2,747.9& \small 4.8
& \small 5,652.6& \small 4.3
& \small 739.9& \small 1.2 \\

& \small \textbf{LW} 
& \small 1,186.7 & \small 10.4
& \small 5,008.1 & \small 10.0
& \small 176.9 & \small 3.5
& \small 340.9 & \small 3.1
& \small 464.5 & \small 4.1
& \small 651.5 & \small 8.3
& \small 1,302.1 & \small 7.1
& \small 849.1 & \small 1.9  \\
\hline

\multirow{1}{{.7cm}}{\small \textbf{DDPG}} 
& \small \textbf{PO} 
& \small 123.3& \small 3.8 
& \small 149.9& \small 2.4
& \small 35.2& \small 2.0
& \small 26.2& \small 1.6 
& \small 39.9& \small 1.8
& \small 165.2& \small 4.8
& \small 78.4& \small 3.3
& \small 25.9& \small 0.6 \\

\hline

\multirow{1}{{.7cm}}{\small \textbf{TD3}} 
& \small \textbf{PO} 
& \small 121.7& \small 5.1 
& \small 206.4& \small 3.2
& \small 30.7& \small 2.7
& \small 26.3& \small 2.1 
& \small 36.2& \small 2.5 
& \small 171.9& \small 6.5
& \small 91.3& \small 4.4
& \small 25.9& \small 0.8 \\
%& \small \textbf{PR} & PC & IOFR  & CODEC & IMAG & IO & COMP & LANG & MATH \\     

%& \small \textbf{LW} & PC & IOFR  & CODEC & IMAG & IO & COMP & LANG & MATH \\   
\hline



\multirow{1}{.33cm}{\small \textbf{SAC}}  
& \small \textbf{PO} 
& \small 144.2& \small 6.6 
& \small 200.5& \small 4.2
& \small 46.7& \small 3.5
& \small 50.2& \small 2.6
& \small 71.6& \small 3.3
& \small 292.4& \small 8.5
& \small 175.8& \small 5.8
& \small 31.1& \small 1.1 \\
\hline
%& \small \textbf{PR} & PC & IOFR  & CODEC & IMAG & IO & COMP & LANG & MATH \\     

%& \small \textbf{LW} & PC & IOFR  & CODEC & IMAG & IO & COMP & LANG & MATH \\   






\multirow{2}{{.7cm}}{\small \textbf{ACKTR}}  
& \small \textbf{PO} 
& \small 117.3& \small 5.8 
& \small 82.7& \small 3.6
& \small 31.6& \small 3.0
& \small 24.6& \small 2.3 
& \small 49.0& \small 2.9
& \small 168.5& \small 7.4
& \small 81.6& \small 5.0
& \small 9.5& \small 0.9 \\

& \small \textbf{PR} 
& \small 826.1& \small 6.6 
& \small 998.9& \small 4.7
& \small 59.5& \small 2.8
& \small 107.2& \small 2.4 
& \small 128.8& \small 3.0
& \small 190.9& \small 6.6
& \small 361.2& \small 5.1
& \small 228.9& \small 1.1 \\

%& \small \textbf{LW} 
%& \small paint  & \small paint 
%& \small iofrol & \small iofrol
%& \small codec & \small 21.3
%& \small IMAG & \small 37.3 
%& \small IO & \small 49.4 
%& \small COMP & \small 126.5
%& \small LANG& \small 122.2
%& \small MATCH& \small 66.6 \\

\hline
\hline





\end{tabular}
\end{center}

\end{table*}
